Robust Stochastic Graph Generator for Counterfactual Explanations

Counterfactual Explanation (CE) techniques have garnered attention as a means to provide insights to the users engaging with AI systems. While extensively researched in domains such as medical imaging and autonomous vehicles, Graph Counterfactual Explanation (GCE) methods have been comparatively under-explored. GCEs generate a new graph similar to the original one, with a different outcome grounded on the underlying predictive model. Among these GCE techniques, those rooted in generative mechanisms have received relatively limited investigation despite demonstrating impressive accomplishments in other domains, such as artistic styles and natural language modelling. The preference for generative explainers stems from their capacity to generate counterfactual instances during inference, leveraging autonomously acquired perturbations of the input graph. Motivated by the rationales above, our study introduces RSGG-CE, a novel Robust Stochastic Graph Generator for Counterfactual Explanations able to produce counterfactual examples from the learned latent space considering a partially ordered generation sequence. Furthermore, we undertake quantitative and qualitative analyses to compare RSGG-CE's performance against SoA generative explainers, highlighting its increased ability to engendering plausible counterfactual candidates.

==> algorithms/sampling.tex <==
\begin{algorithm}[!t]
\caption{Iterative sampling edges to produce a counterfactual.}\label{algo:sampling}
\begin{algorithmic}[1]
\Require$G_* = (X_*,A_*)$, $\mathbb{G}:\mathcal{G} \rightarrow \mathcal{G}$, $k \in \mathbb{N}_+$, $\Phi$, 
\State $G' \gets \emptyset$
\State $\hat{A}_*, Z_* = \mathbb{G}(A_*,X_*)$\Comment{\textit{Generate a new adjacency tensor $\hat{A}_*$ and new node representations $Z$}}
\State $V_i, V_j \gets (A \neq 0)$ \Comment{\textit{Get the vertices where there are edges}}
\State $A' \gets \texttt{sample}(V_i,V_j,\hat{A}, \texttt{num\_samples=}|V_i|\times |V_j|)$\Comment{\textit{Sample (with replacement) $|V_i| \times |V_j|$ edges from the original edges according to the estimated edge probabilities $\hat{A}$}}
\State $G' \gets (Z',A')$
\If{$\Phi(G_*) \neq \Phi(G')$}
    \State \Return $G'$
\Else
    \While{$k \geq 0$}
        \State $V_i,V_j \gets (A' = 0)$ \Comment{\textit{Get the vertices where there are no edges (i.e. negative edges)}}
        \State $A' \gets A' \cup \texttt{uniform}(V_i\times V_j)$\Comment{\textit{Uniformly sample one edge from $V_i \times V_j$}}
        \State $G^\prime \gets (Z',A')$

        \State $k \gets k - 1$
        \If{$\Phi(G_*) \neq \Phi(G')$}
            \State \Return $G'$
        \EndIf
    \EndWhile
    
\EndIf
\State \Return $G_*$ \Comment{\textit{Sampling a valid counterfactual failed}}
\end{algorithmic}
\label{algo:irand}
\end{algorithm}

==> tables/datasets.tex <==
\begin{table}[h]
\centering
\caption{Statistical description of the datasets.}
\label{tab:gr_datasets}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lrrr@{}}
\toprule
Dataset            & Tree-Cycles   & ASD  \\ \midrule
\# of instances    &  500          & 101   \\
Avg graph diameter & 12.812        & $\infty$ \\
Avg \# of nodes    & 28            & 116          \\
Avg \# of edges    & 27.566        & 655.624     \\
Max \# of nodes    & 28            & 116        \\
Avg node degree    & 1.969         & 11.304        \\ 
\# of classes      & 2             & 2         \\
Class distribution & 0.504 : 0.496 & 0.515 : 0.485        \\
Graph type         & Undirected    & Undirected \\
Connected components & One & Multiple\\
 \bottomrule
\end{tabular}%
}
\end{table}

==> tables/tab_hyperparameters.tex <==
\begin{table*}[!ht]
\centering
\caption{Hyperparameters of the methods.}
\label{tab:hyperparams}
\begin{tabular}{llllllllllll|ll}
\hline
Method & Ep & Batch Size & lr & $\alpha$ & $\lambda$ & $\gamma$ & Dropout & Weight Decay & $\lambda_{sim}$ & $\lambda_{kl}$ & $\lambda_{cfe}$ & GED    & Validity \\
\hline
$CF^2$ & 500    & 0.2        & 0.01          & 0.7    & 20      & 0.9    & -       & -            & -            & -            & -             & 27.58  & 0.5      \\
CLEAR  & 50     & 0.1        & 0.0001        & 0      & -       & -      & 0       & 0.0001       & 0.1          & 0.1          & 0.1           & 117.35 & 0.5\\
\hline
\end{tabular}
\end{table*}
